Learning to Balance: Bayesian Meta-Learning for Imbalanced and Out-of-distribution Tasks

While tasks could come with varying the number of instances and classes in realistic settings, the existing meta-learning approaches for few-shot classification assume that the number of instances per task and class is fixed. Due to such restriction, they learn to equally utilize the meta-knowledge across all the tasks, even when the number of instances per task and class largely varies. Moreover, they do not consider distributional difference in unseen tasks, on which the meta-knowledge may have less usefulness depending on the task relatedness. To overcome these limitations, we propose a novel meta-learning model that adaptively balances the effect of the meta-learning and task-specific learning within each task. Through the learning of the balancing variables, we can decide whether to obtain a solution by relying on the meta-knowledge or task-specific learning. We formulate this objective into a Bayesian inference framework and tackle it using variational inference. We validate our Bayesian Task-Adaptive Meta-Learning (Bayesian TAML) on multiple realistic task- and class-imbalanced datasets, on which it significantly outperforms existing meta-learning approaches. Further ablation study confirms the effectiveness of each balancing component and the Bayesian learning framework.

==> ablation_table.tex <==
\begin{table}[h]
	\caption{\small \textbf{Ablation Study for effectiveness of \hy{Bayesian} learning and statistics.} All reported results are average performances over 600 randomly selected episodes with standard errors for 95\% confidence interval over tasks. The number of gradient steps is set to $3$ for all models.
	}\label{tbl:ablation}
	\small
	\begin{center}
		\begin{tabular}{cc}
			\toprule
			Models & Imbal. t-ImgNet ($K$=5) \\
			\hline
			\hline
			Meta-SGD					& 67.18 $\pm$ 0.74 \\
			Deterministic TAML			& xx.xx $\pm$ x.xx \\
			$\bs\gamma_\ts$- Bayesian	& xx.xx $\pm$ x.xx \\
			$\bz_\ts$- Bayesian			& xx.xx $\pm$ x.xx \\			
			BayesianTCAML				& \bf71.73 $\pm$ 0.39 \\
			\bottomrule
		\end{tabular}
		\hspace{0.5 in}
		\begin{tabular}{cc}
			\toprule
			Models & Imbal. t-ImgNet ($K$=5) \\
			\hline
			\hline
			Mean			& 68.63 $\pm$ 0.39 \\
			Variance		& 69.98 $\pm$ 0.37 \\
			Skewness		& 70.31 $\pm$ 0.38 \\
			Kurtosis		& 71.06 $\pm$ 0.41 \\			
			Full Stat.		& \bf71.73 $\pm$ 0.39 \\
			\bottomrule
		\end{tabular}
	\end{center}
	\small

\end{table}

==> fewshot_table.tex <==

\begin{savenotes}
\begin{table}[ht]
	\begin{center}
		\vspace{-0.15in}
		%\caption{\small \textbf{Few-shot classification performance.} All reported results are average performances over 1000 for Omniglot and 600 for mini-ImageNet randomly selected episodes with standard errors for 95\% confidence interval over tasks.}\label{tbl:fsl}
		%\vspace{-0.05in}
		\small
		\resizebox{1.0\textwidth}{!}{
			\begin{tabular}{ccccc}
				\toprule
				&\multicolumn{2}{c}{Omniglot 20-way} & \multicolumn{2}{c}{mini-ImageNet 5-way} \\\cmidrule{1-5}
				Models & 1-shot & 5-shot & 1-shot & 5-shot \\
				\hline
				\hline
				Meta-Learner LSTM \cite{ravi2016optimization}& - & - & 43.44 \tiny $\pm$ 0.77 & 60.60 \tiny $\pm$ 0.71 \\
				Prototypical Networks \cite{snell2017prototypical} \footnote{We adopt the accuracies of the Prototypical Network in the setting which the number of shot and way are the same for training and testing phase for the consistency with other methods. In the "higher way" setting where 20-way is used during training for 5-way testing, the reported performance of the model is 68.20 $\pm$ 0.66\%.} & 96.0 & 98.9 & 49.42 \tiny $\pm$ 0.78 & 65.77 \tiny $\pm$ 0.70 \\			
				%\hline
				MAML \citep{finn2017model}			  & 95.80 \tiny$\pm$ 0.30 	  & 98.90 \tiny$\pm$ 0.20     & 48.70  \tiny$\pm$ 1.84    & 63.11 \tiny $\pm$ 0.92 \\
				Meta-SGD \citep{li2017meta} 		  & 95.93 \tiny$\pm$ 0.38 	  & 98.97 \tiny$\pm$ 0.19 	  & 50.71 \tiny$\pm$ 1.87 	  & 64.03 \tiny $\pm$ 0.94 \\
				Meta-SGD ($K$=3,5)					  & 96.03 \tiny$\pm$ 0.43 	  & 98.72 \tiny$\pm$ 0.56 	  & 49.63 \tiny$\pm$ 1.41 	  & 63.74 \tiny$\pm$ 1.03 \\
				Relation Net \citep{yang2017learning} & 97.60 \tiny$\pm$ 0.20 	  & 99.10 \tiny$\pm$ 0.10 	  & 50.44 \tiny$\pm$ 0.82  	  & 65.32 \tiny$\pm$ 0.70 \\
				MT-NET \citep{lee2018gradient}		  & 96.20 \tiny$\pm$ 0.40 	  & - 						  & 51.70 \tiny$\pm$ 1.84     & - \\
				Probabilistic MAML \citep{prob_maml}  & - 						  & - 						  & 50.13 \tiny$\pm$ 1.86  	  & - \\
				Reptile \citep{nichol2018first}		  & 89.43 \tiny$\pm$ 0.14 	  & 97.12 \tiny$\pm$ 0.32 	  & 49.97 \tiny$\pm$ 0.32  	  & 65.99 \tiny$\pm$ 0.58 \\
				BMAML \citep{kim2018bayesian} 		  & -				 		  & -			 			  & \bf 53.80 \tiny$\pm$ 1.46 & -				 \\
				VERSA \citep{gordon2018meta}		  & 97.66 \tiny$\pm$ 0.29 	  & 98.77 \tiny$\pm$ 0.18 	  & 53.40 \tiny$\pm$ 1.82 	  &  67.37 \tiny$\pm$ 0.86 \\
				\hline
				Bayesian TAML						  & \bf 98.10 \tiny$\pm$ 0.26 & \bf 99.12 \tiny$\pm$ 0.18 & 51.72 \tiny$\pm$ 1.62 	  & \bf 68.32 \tiny$\pm$ 1.11 \\
				\bottomrule	
			\end{tabular}
		}
		\vspace{-0.15in}
	\end{center}
	\small
\end{table}
\end{savenotes}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> minimeta_table.tex <==
\begin{table}[h]
	\vspace{-0.1in}
	\caption{\small \textbf{Imbalanced Few-shot classification performance on \textsc{MiniMeta Dataset}.} The models are trained wtih the former 8 datasets with realistic imbalance setting (Traffic Signs and MSCOCO are evaluated only). All reported results are averaged performances over 600 randomly selected episodes for each dataset with standard errors for 95\% confidence intervals. 
		%ID denotes datasets used during meta-training and OOD denotes datasets not seen during meta-training.
	}\label{tbl:analysis_minimeta}
	\vspace{-0.06in}
	\small
	\begin{center}
		\begin{tabular}{cccccc}
			\toprule
			Test Source 	  & Finetune & Prototypical Net  & fo-MAML   & Proto-MAML & Bayesian-TCAML \\
			\hline
			\hline
			ILSVRC		  & 14.81 $\pm$ 0.63 & 30.12 $\pm$ 1.00 & 18.02 $\pm$ 0.64 &31.90 $\pm$ 1.02 & x $\pm$ x \\
			Omniglot   	  & 64.50 $\pm$ 1.36 & 84.45 $\pm$ 0.92 & 76.37 $\pm$ 0.99 &91.16 $\pm$ 0.63 & x $\pm$ x \\
			Aircraft  	  & 35.67 $\pm$ 1.04 & 61.28 $\pm$ 1.10 & 61.18 $\pm$ 0.91 &74.49 $\pm$ 0.93 & x $\pm$ x \\
			Birds		  & 25.54 $\pm$ 1.09 & 56.50 $\pm$ 1.16 & 47.22 $\pm$ 1.11 &64.67 $\pm$ 0.99 & x $\pm$ x \\
			Textures      & x $\pm$ x & 55.02 $\pm$ 1.05 & 42.99 $\pm$ 0.95 &52.18 $\pm$ 0.99 & x $\pm$ x \\
			Quick Draw	  & x $\pm$ x & 63.86 $\pm$ 1.04 & 51.18 $\pm$ 1.12 &69.40 $\pm$ 1.02 & x $\pm$ x \\
			Fungi 		  & x $\pm$ x & 37.94 $\pm$ 0.91 & 29.20 $\pm$ 0.98 &45.38 $\pm$ 1.12 & x $\pm$ x \\
			VGG Flower    & x $\pm$ x & 76.21 $\pm$ 0.76 & 58.06 $\pm$ 1.10 &76.73 $\pm$ 1.11 & x $\pm$ x \\
			Traffic Signs & x $\pm$ x & 45.32 $\pm$ 1.05 & 29.64 $\pm$ 1.04 &42.49 $\pm$ 1.11 & x $\pm$ x \\
			MSCOCO 		  & x $\pm$ x & 31.87 $\pm$ 1.04 & 17.92 $\pm$ 0.79 &28.76 $\pm$ 1.04 & x $\pm$ x \\			
			\bottomrule
		\end{tabular}
	\end{center}
	\small
	\label{tbl:analysis_minimeta}
	\vspace{-0.15in}
\end{table}


\iffalse
\begin{table}[h]
	\vspace{-0.1in}
	\caption{\small \textbf{Realistic few-shot classification performance on Mini-Meta-Dataset.} The models are trained wtih all dataset with realistic imbalance setting. All reported results are averaged performances over 600 randomly selected episodes for each dataset with standard errors for 95\% confidence intervals. 
	%ID denotes datasets used during meta-training and OOD denotes datasets not seen during meta-training.
	}\label{tbl:analysis_minimeta}
	\vspace{-0.06in}
	\small
	\begin{center}
		\begin{tabular}{ccccccc}
			\toprule
			Test Source 	  & \textit{k}-NN & Finetune & Prototypical Net  & fo-MAML   & Proto-MAML & Bayesian-TAML \\
			\hline
			\hline
				ILSVRC		  & x $\pm$ x & x $\pm$ x & x $\pm$ x &x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
				Omniglot   	  & x $\pm$ x & x $\pm$ x & x $\pm$ x &x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
				Aircraft  	  & x $\pm$ x & x $\pm$ x & x $\pm$ x &x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
				Birds		  & x $\pm$ x & x $\pm$ x & x $\pm$ x &x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
				Textures      & x $\pm$ x & x $\pm$ x & x $\pm$ x &x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
				Quick Draw	  & x $\pm$ x & x $\pm$ x & x $\pm$ x &x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
				Fungi 		  & x $\pm$ x & x $\pm$ x & x $\pm$ x &x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
				VGG Flower    & x $\pm$ x & x $\pm$ x & x $\pm$ x &x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
				Traffic Signs & x $\pm$ x & x $\pm$ x & x $\pm$ x &x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
				MSCOCO 		  & x $\pm$ x & x $\pm$ x & x $\pm$ x &x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
			\hline
			\hline
				Avg. rank 	  & x 		  & x 		  & x 	 	  &x 		 & x          & x \\			
			\bottomrule
		\end{tabular}
	\end{center}
	\small
	\label{tbl:analysis_minimeta}
	\vspace{-0.15in}
\end{table}
\fi

\iffalse
\begin{table}[h]
	\vspace{-0.1in}
	\caption{\small \textbf{Realistic few-shot classification performance on MiniMeta-Dataset.} The models are trained with Omniglot (left) and tiered-ImageNet (right) with imbalance setting. All reported results are averaged performances over 1000 and 600 randomly selected episodes for each dataset with standard errors for 95\% confidence intervals. 
		%ID denotes datasets used during meta-training and OOD denotes datasets not seen during meta-training.
	}\label{tbl:analysis_minimeta}
	\vspace{-0.08in}
	\small
	\begin{center}
		\begin{tabular}{ccccccccccc}
			\toprule
			Test Source 	  & ILSVRC  & Omniglot   & Aircraft & Birds & Textures & Quick Draw & Fungi & VGG Flower & Traffic Signs & MSCOCO \\
			\hline
			\hline
			ProtoNet		  & x       & x          & x        & x     &x         & x          & x     & x          &x              & x   \\
			%fo-MAML   	  & x $\pm$ x & x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
			%Proto-MAML  	  & x $\pm$ x & x $\pm$ x & x $\pm$ x  & x $\pm$ x\\
			%B-TAML	  & x $\pm$ x & x $\pm$ x & x $\pm$ x  & x $\pm$ x\\

			\bottomrule
		\end{tabular}
	\end{center}
	\small
	\label{tbl:analysis_minimeta}
	\vspace{-0.15in}
\end{table}
\fi

==> supplementary_table.tex <==
\begin{table}[h]
	%\vspace{-0.1in}
	\small
	\begin{center}
		\begin{tabular}{ccc|cc}
			\toprule
			Models ($K$=5) 				 & Omniglot 				 & MNIST 					& tiered-ImageNet 			& mini-ImageNet\\
			\hline
			\hline
			Bayesian TAML (Naive approx.) & 96.18 	 \tiny$\pm$ 0.33 & 83.95    \tiny$\pm$ 0.52 & 71.17     \tiny$\pm$ 1.09 & 57.68    \tiny$\pm$ 0.48\\
			Bayesian TAML (MC approx.)	  & \bf96.29 \tiny$\pm$ 0.31 & \bf84.39 \tiny$\pm$ 0.48 & \bf 71.42 \tiny$\pm$ 1.00 & \bf58.37 \tiny$\pm$ 0.49\\
			\bottomrule
		\end{tabular}
	\end{center}
	\small
	\caption{\small \textbf{Classification performance under realistic scenario.} The models are trained with Omniglot(left) and tiered-ImageNet(right) with imbalanced setting. All reported results are average performances over 1000 for Omniglot and MNIST and 600 for tiered-ImageNet and mini-ImageNet randomly selected episodes with standard errors for 95\% confidence interval over tasks.}\label{tbl:analysis_spl}
	\vspace{-0.08in}
\end{table}

==> z_init_table.tex <==
\begin{wraptable}{r}{8cm}
	\vspace{-0.2in}
	\begin{center}
		\resizebox{0.55\textwidth}{!}{
			\small
		\begin{tabular}{ccc}
	\toprule
	%Meta-train & \multicolumn{2}{c}{Omniglot + VGG flower + DTD (OVD)}  \\
	%\hline
	Meta-test (5-way 10-shot) & Omniglot & MNIST \\
	\hline
	\hline
%	Meta-SGD			  & 98.38 \tiny$\pm$ 0.23   & 90.42 \tiny$\pm$ 0.28\\
	Bayesian g(z) TAML + Interpolation & 98.83 \tiny$\pm$ 0.08 & 92.03 \tiny$\pm$ 0.19 \\
	Bayesian g(z) TAML		  & \bf98.92 \tiny$\pm$ 0.30 & \bf92.06 \tiny$\pm$ 0.32\\
	\bottomrule
	\vspace{-0.2in}
\end{tabular}
		}
	\end{center}
	\vspace{-0.12in}
	\caption{\small \textbf{ Classification results to $\theta_0$ inititalization with  $g(z)$.}}\label{tbl:interpolation}
	%All reported results are averaged performances over 1000 and 600 randomly selected episodes for each dataset with standard errors for 95\% confidence intervals
	\vspace{-0.1in}
\end{wraptable}



